Test-Time Training on Video Streams

Prior work has established Test-Time Training (TTT) as a general framework to further improve a trained model at test time. Before making a prediction on each test instance, the model is first trained on the same instance using a self-supervised task such as reconstruction. We extend TTT to the streaming setting, where multiple test instances - video frames in our case - arrive in temporal order. Our extension is online TTT: The current model is initialized from the previous model, then trained on the current frame and a small window of frames immediately before. Online TTT significantly outperforms the fixed-model baseline for four tasks, on three real-world datasets. The improvements are more than 2.2x and 1.5x for instance and panoptic segmentation. Surprisingly, online TTT also outperforms its offline variant that accesses strictly more information, training on all frames from the entire test video regardless of temporal order. This finding challenges those in prior work using synthetic videos. We formalize a notion of locality as the advantage of online over offline TTT, and analyze its role with ablations and a theory based on bias-variance trade-off.

==> jmlr_coverletter.tex <==
% !TEX program = pdflatex
\input{jmlr_coverletter_preamble.tex}

\begin{document}
\hfill{\today}

Journal of Machine Learning Research

\bigskip

Dear Editors:

We are writing to submit our manuscript ``Test-Time Training in Video Sreams'' to the \emph{Journal of Machine Learning Research}.

This paper extends our work of ``Test-Time Training with Masked Autoencoders'', published at NeurIPS 2022. Our submission significantly extends beyond the original NeurIPS paper in the following ways:

\textbf{New setting and applications}.
Our submission considers video frames, with temporal smoothness, from one stream at a time. 
The conference paper only considers independent images from datasets like ImageNet. 
To make meaningful evaluations in the streaming setting, we also consider four new applications: semantic, instance and panoptic segmentation, as well as colorization. The conference paper only considers object recognition.

\textbf{New insights and empirical results}.
Given the temporal dimension in our new setting, we can now ask:
\emph{Is training on the future once it actually happens better than training on all possible futures in advance?}
We formulate this question concretely, and answer it rigorously through empirical results. This answer gives us new insights on generalization with test-time training, about the important role of \textbf{locality}.

\textbf{New theoretical results}. Our new theory in Section 6.2 explains our empirical results on locality, saying that forgetting can be beneficial for test-time training in video streams. 

We suggest the following action editors and referees for our submission.

Action Editors:
\begin{itemize}
    \item Samy Bengio, Apple, bengio@apple.com
    \item George Konidaris, Duke University, gdk@cs.brown.edu
    \item Honglak Lee, University of Michigan, honglak@eecs.umich.edu
    \item Ruslan Salakhutdinov, Carnegie Mellon University, rsalakhu@cs.cmu.edu
    \item Fei Sha, Google, fsha@google.com
    \item Kilian Weinberger, Cornell University, kilian@cornell.edu
\end{itemize}

Reviewers:
\begin{itemize}
    \item David Duvenaud, University of Toronto, duvenaud@cs.toronto.edu
    \item Roger Grosse, University of Toronto, rgrosse@cs.toronto.edu
    \item Zachary Lipton, Carnegie Mellon University, zlipton@cmu.edu
    \item Chiyuan Zhang, Google Research, pluskid@gmail.com
    \item Andrew Gordon Wilson, New York University, andrewgw@cims.nyu.edu
    \item Hao Li, Amazon AGI / AWS AI Labs, hao.li.ict@gmail.com
\end{itemize}

Our submission has the following keywords: \textbf{deep learning, computer vision, test-time training}.

As the corresponding author, I confirm that none of the co-authors listed below have a conflict of interest with the action editors and referees I suggest above. Further, I confirm that all co-authors below consent to my submission of this manuscript to the \emph{Journal of Machine Learning Research}.

\bigskip

Sincerely,

\medskip

Renhao Wang, UC Berkeley\\
Yu Sun, UC Berkeley\\
Yossi Gandelsman, UC Berkeley\\
Xinlei Chen, Meta\\
Alexei A. Efros, UC Berkeley\\
Xiaolong Wang, UC San Diego\\
\end{document}








































==> jmlr_revision_cover.tex <==
% !TEX program = pdflatex
\input{jmlr_coverletter_preamble.tex}

\begin{document}
\hfill{\today}

Journal of Machine Learning Research

\bigskip

Dear Editors:

Thank you very much for accepting our paper subject to minor revisions. We have carefully read the reviews and addressed all the concerns.

\begin{quote}
\textit{
...a discussion about hyper-parameter settings, given some recent criticisms of the overall approach...
}
\end{quote}
The reviewer is specifically questioning the ``influence of the sliding window size on performance, as shown in Figure 5.'' We have added discussion about the window size $k$ in the caption of the figure. 
Note that the x-axis here is in log scale, in order to highlight the effect of $k$ over a large range. Performance is actually not sensitive to $k$ in linear scale.


\begin{quote}
\textit{
...more information about the efficiency of the method would be valuable (time and memory) even if this was not the focus of the paper...
}
\end{quote}
Table 1 now contains the time per frame using a single A100 GPU for every method, including \emph{Offline TTT-MAE All Frames}. The caption of Table 1, as well as the end of Subsection 5.2, discusses the time above.

\begin{quote}
\textit{
...consider in-context learning as well.
}
\end{quote}
We have expanded Section 7 significantly to discuss the relationship between our method and in-context learning.

Thank you again for your feedback!

\bigskip

Sincerely,

\medskip

Renhao Wang, UC Berkeley\\
Yu Sun, UC Berkeley\\
Arnuv Tandon, Stanford University\\
Yossi Gandelsman, UC Berkeley\\
Xinlei Chen, Meta\\
Alexei A. Efros, UC Berkeley\\
Xiaolong Wang, UC San Diego\\
\end{document}

